A Catalog of Galaxies behind the Southern Milky Way. - I. The Hydra/Antlia Extension (l: 266 - 296 deg)

A deep optical galaxy search in the southern Milky Way - aimed at reducing the width of the Zone of Avoidance - revealed 3279 galaxy candidates above the diameter limit of D > 0.2 arcmin, of which only 112 (3.4%) were previously catalogued. The surveyed region (266 < l < 296 and -10 < b < +8) lies in the extension of the Hydra and Antlia clusters - where a supercluster is suspected - and in the approximate direction of the dipole anisotropy in the Cosmic Microwave Background radiation. Here we present the optical properties of the unveiled galaxies such as positions, diameters, magnitudes, morphological types, including a detailed discussion on the quality of these data and the completeness limits as a function of the foreground dust extinction. For 127 of the 227 positional matches in the IRAS PSC, a reliable cross-identification could be found. Several distinct overdensities and filaments of galaxies can be identified that are apparently uncorrelated with the Galactic foreground extinction hence the probable signature of extragalactic large-scale structures. This catalog constitutes the first part in a series of five equally conducted optical searches for galaxies in the southern Milky Way (245 < l < 350). With these surveys, the entire Zone of Avoidance will have been covered by means of visual inspection. The catalogs build the basis for various spectroscopic and photometric follow-up programs which eventually will allow a thorough analyse of the galaxy distribution in redshift space and the peculiar velocity fields within the Zone of Avoidance, as well an an improved understanding of the Galactic foreground extinction.

==> header.tex <==
 \end{tabular*}
 \normalsize
 \end{table*}
\addtocounter{table}{-1}
\clearpage
%\newpage

\begin{table*}
 \normalsize
 \renewcommand{\baselinestretch}{0.6}
\caption{Galaxies in the southern ZOA -- I.  The Hydra/Antlia
 Extension (continued)}
\scriptsize
\begin{tabular*}{18cm}{ 
%@{\extracolsep\fill}
  r  @{\extracolsep{1mm}} p{1.2cm} @{\extracolsep{1mm}} 
% 1                       2                      
% RKK                     Other                   
  p{4mm} @{\extracolsep{1mm}}  
% 3
% IR
  l@{\extracolsep{2mm}} l @{\extracolsep{3mm}}
% 4                       5
% RA                      Dec
  r @{\extracolsep{2mm}}r @{\extracolsep{2mm}} r @{\extracolsep{2mm}}
% 6                     7                      8  
% gal l                 gal b                  SRC
  r @{\extracolsep{2mm}}    r @{\extracolsep{3mm}} 
% 9                        10                    
% X                        Y                     
  p{6mm} @{\extracolsep{0mm}} p{4.5mm} @{\extracolsep{2mm}}
% 11
% Dx                     d
  r @{\extracolsep{2mm}} r @{\extracolsep{2.5mm}} l @{\extracolsep{1mm}} 
%  12                   13                     14 
%  Bj                   HI                     U
  p{2.7mm} @{\extracolsep{-1mm}} p{2.7mm} @{\extracolsep{-1mm}} 
  p{2.7mm} @{\extracolsep{-1mm}} 
  p{2.7mm} @{\extracolsep{-0.5mm}} p{2.7mm} @{\extracolsep{0mm}} 
% 15a-e      
% T1-5
  p{2.7mm} @{\extracolsep{-0.5mm}} p{2.7mm} @{\extracolsep{0mm}} 
% 15f-g      
% T f-g
  l }
%   16
%   Remarks
\hline 
\vspace{-1mm} \\
 RKK & Other & IR & \ \ \ \ R.A. & \ \ \ Dec.& gal $\ell$ \ & gal $b \ $ 
 & SRC & X \ \ & Y \ \ & 
% \multicolumn{2}{c}{D x d}& $B_{\rm J}$ & N$_{\rm HI}$ &  & 
 \multicolumn{2}{c}{D x d}& $B_{J}$ & N$_{HI}$ &  & 
 \multicolumn{5}{c}{Type} &&& Remarks \\
 Ident & Ident &  &(h\,\, m\,\, s) & ($\deg$\,\, $\arcmin$\,\,
 $\arcsec$) & ($\deg$) \ &($\deg$) \ 
%  & & (mm) & (mm) & \multicolumn{2}{c}{($\arcsec$)} & ($^{\rm m})$ & &
  & & (mm) & (mm) & \multicolumn{2}{c}{($\arcsec$)} & ($^{m})$ & &
  u & \multicolumn{5}{c}{class.} &o &* & \\
\vspace{-1mm} \\
 (1) & (2) & (3) & \ \ \ \ (4) & \ \ \ \ (5) & (6) \ & (7) \ 
 & (8) & (9) \ & (10) \ &
 \multicolumn{2}{c}{(11)} & (12) & (13) & & \multicolumn{5}{c}{(14)} 
 &&& (15)\\
\vspace{-1mm} \\
\hline 
\vspace{-1mm} \\




==> header_end.tex <==
\vspace{-1.3 mm} \\ 
\hline
\end{tabular*}
\normalsize
\label{cat}
\end{table*}






==> header_start.tex <==
\begin{table*}
 \normalsize
 \renewcommand{\baselinestretch}{0.6}
\caption{Galaxies in the southern ZOA -- I.  The Hydra/Antlia Extension}
% \label{tab1}
\scriptsize
\begin{tabular*}{18cm}{ 
%@{\extracolsep\fill}
  r  @{\extracolsep{1mm}} p{1.2cm} @{\extracolsep{1mm}} 
% 1                       2                      
% RKK                     Other                   
  p{4mm} @{\extracolsep{1mm}}  
% 3
% IR
  l@{\extracolsep{2mm}} l @{\extracolsep{3mm}}
% 4                       5
% RA                      Dec
  r @{\extracolsep{2mm}}r @{\extracolsep{2mm}} r @{\extracolsep{2mm}}
% 6                     7                      8  
% gal l                 gal b                  SRC
  r @{\extracolsep{2mm}}    r @{\extracolsep{2.5mm}} 
% 9                        10                    
% X                        Y                     
  p{6mm} @{\extracolsep{0mm}} p{4.5mm} @{\extracolsep{2mm}}
% 11
% Dx                     d
  r @{\extracolsep{2mm}} r @{\extracolsep{2.5mm}} l @{\extracolsep{1mm}} 
%  12                   13                     14 
%  Bj                   HI                     U
  p{2.7mm} @{\extracolsep{-1mm}} p{2.7mm} @{\extracolsep{-1mm}} 
  p{2.7mm} @{\extracolsep{-1mm}} 
  p{2.7mm} @{\extracolsep{-0.5mm}} p{2.7mm} @{\extracolsep{0mm}} 
% 15a-e      
% T1-5
  p{2.7mm} @{\extracolsep{-0.5mm}} p{2.7mm} @{\extracolsep{0mm}} 
% 15f-g      
% T f-g
  l }
%   16
%   Remarks
\hline 
\vspace{-1mm} \\
 RKK & Other & IR & \ \ \ \ R.A. & \ \ \ Dec.& gal $\ell$ \ & gal $b \ $ 
 & SRC & X \ \ & Y \ \ & 
% \multicolumn{2}{c}{D x d}& $B_{\rm J}$ & N$_{\rm HI}$ &  & 
 \multicolumn{2}{c}{D x d}& $B_{J}$ & N$_{HI}$ &  & 
 \multicolumn{5}{c}{Type} &&& Remarks \\
 Ident & Ident &  &(h\,\, m\,\, s) & ($\deg$\,\, $\arcmin$\,\,
 $\arcsec$) & ($\deg$) \ &($\deg$) \ 
%  & & (mm) & (mm) & \multicolumn{2}{c}{($\arcsec$)} & ($^{\rm m})$ & &
  & & (mm) & (mm) & \multicolumn{2}{c}{($\arcsec$)} & ($^{m})$ & &
  u & \multicolumn{5}{c}{class.} &o &* & \\
\vspace{-1mm} \\
 (1) & (2) & (3) & \ \ \ \ (4) & \ \ \ \ (5) & (6) \ & (7) \ 
 & (8) & (9) \ & (10) \ &
 \multicolumn{2}{c}{(11)} & (12) & (13) & & \multicolumn{5}{c}{(14)} 
 &&& (15)\\
\vspace{-1mm} \\
\hline 
\vspace{-1mm} \\

